Achieving Multi-Port Memory Performance on Single-Port Memory with Coding Techniques

Many performance critical systems today must rely on performance enhancements, such as multi-port memories, to keep up with the increasing demand of memory-access capacity. However, the large area footprints and complexity of existing multi-port memory designs limit their applicability. This paper explores a coding theoretic framework to address this problem. In particular, this paper introduces a framework to encode data across multiple single-port memory banks in order to {\em algorithmically} realize the functionality of multi-port memory. This paper proposes three code designs with significantly less storage overhead compared to the existing replication based emulations of multi-port memories. To further improve performance, we also demonstrate a memory controller design that utilizes redundancy across coded memory banks to more efficiently schedule read and write requests sent across multiple cores. Furthermore, guided by DRAM traces, the paper explores {\em dynamic coding} techniques to improve the efficiency of the coding based memory design. We then show significant performance improvements in critical word read and write latency in the proposed coded-memory design when compared to a traditional uncoded-memory design.

==> abstract.tex <==
Memory systems work hard to keep up with access requests from cores. Growing computer sizes, heterogeneous systems and increasing level of integration has increased more. Performance focused systems use enhancements like multi-port memories to increase the access capacity. However, they come with a cost in terms of area, complexity and cost of redesign and rebuilding a system. In this paper, we explore a mathematical solution to the problem where we explore an efficient memory storage and reterival mechanism for efficent access. We first analyze the request pattern of general memory controller and a application-specific memory controller. \\
We then provide a mathematical approach to storing the data in specific way to achieve higher access rate. We call this specific way of storing the memory as Algorithmic Memory. We discuss methods to design codes and provide example designs for 8 bank memory systems. \\
At last, we analyze and compare the improvement of coded memory with general memory. We present a significant improvement in critical word read and write latency with coded memory. We also provide intuitions derived from this analysis which can help the system designers to efficiently use Algorithmic memory implementation. 

==> app_code_design.tex <==
\section{Code Design Objectives}

The following objects inspired our proposed memory system:
\begin{itemize}
\item Read access : 4 per bank in one cycle
\item Write access : 2 per bank in one cycle
\item Shared Memory size 8 kB - 256 kB
\item Number of Banks : 8
\item Memory overhead : 15$ \% $
\item Parity banks : 5 or 6 shallow banks for code storage
\end{itemize}



==> app_motivation.tex <==
\section{Motivation for Dynamic Coding}\label{sec:parsec_motivation}
%\subsubsection{Motivation}
Bank conflicts are most likely to occur when regions of shared memory are localized to certain memory regions. Multi-core systems often generate memory access requests to overlapping memory regions. By dynamically coding certain memory locales, the proposed memory system aims to resolve the bank conflicts which occur during periods of heavy memory access in multi-core systems.

\begin{figure}[htbp]
		\includegraphics[width=\linewidth]{fig/dedup_whole.png}
		\caption{\it{Memory Access from the Dedup PARSEC benchmark. This trace was generated using 8 cores.}}
		\label{fig:dedup_whole}
\end{figure}

\begin{figure}[htbp]
		\includegraphics[width=\linewidth]{fig/dedup_dense.png}
		\caption{\it{Memory Access from the Dedup PARSEC benchmark demonstrating the density of memory accesses}}
		\label{fig:dedup_dense}
\end{figure}

An examination of the memory trace from one of the PARSEC benchmarks illustrates a scenario where dynamic coding works well. Figure~\ref{fig:dedup_whole} shows the memory trace of a simulation of an 8-core system running the dedup PARSEC benchmark. The y-axis shows the address accessed by the cores. The x-axis shows the access time in nanoseconds. This plot shows that most of the accesses from various cores are primarily located in the lower memory band. Greater than 95\% of all memory accesses are in this band. Figure~\ref{fig:dedup_dense} magnifies this band and reveals that the lower band is composed of two sub-bands of roughly equal density. In a scenario where the dynamic coder can choose to encode two memory blocks it would detect that nearly all memory access are localized to the primary memory bands, so only those regions would be encoded.


Figure~\ref{fig:dedup_dense} shows that the dedup benchmark contains very dense memory utilization. Across all processors, there is an average of $1.11$ ns between accesses per core. This implies an average of $2.22$ cycles between memory access requests per $2$ Ghz processor. Crucially, the most heavily used memory regions are stationary with respect to time for all PARSEC benchmarks. 

Figure~\ref{fig:dedup_whole} shows an entire dedup memory trace. There are two major bands clearly visible in this image, and the bands stay in the same memory regions for the entirety of the trace. Figure~\ref{fig:dedup_dense} is a magnified view of the bottom band. This figure reveals that the bottom band is composed of two sub-bands which are also stationary with respect to time. The structure of the dedup the memory trace is representative for all the PARSEC benchmarks. It is also clear from this image that the memory regions utilized by all of the processors overlap sufficiently to create bank conflicts.



==> sysCResults.tex <==
% This file contains all the results ran on sysC Implementation of the scheme.
\cleardoublepage
\section{SystemC implementation Results}
This section describes the performance results for simulation of code designs on 
systemC platform. We implement system C model of the memory controller with code 
design 1 as described in figure 3. The model is used as a simulator with input 
as memory access traces. The simulator logs the latency of each memory request. 
\\ 
The traces are essentially a list of access requests with a field for time. These request act as command to the memory controller. \\
The performance charts for each traces comprise of four metrics as described 
below. 
\begin{itemize}
	\item {\bf Critical Read Latency} This parameter is the average latency 
		experienced by the most critical word of a read request. This 
		metric is averaged over the whole execution of the trace. 
		Evident from its name, critical word releases the processor from 
		the stall and the other memory elements in the cache line can 
		follow it. The critical read latency is calculated by taking an 
		average of critical read latency of all the requests from all 6 cores. 
	\item {\bf Transactional Read Latency} is the latency of the whole read 
		memory request. This is also averaged over the whole execution 
		of the trace, i.e., over requests from all the cores. This determines 
		the average latency of read accesses.
	\item {\bf Write Latency} is the measure of average latency of write 
		requests before it is committed to the memory. This does not 
		account for the latency caused by reCoding. Since the cost of 
		recoding is embedded in the cost of future read/writes. The 
		average is taken over all the requests received by the memory 
		controller over all the cores.
	\item {\bf Trace Execution time} is the time taken to process a trace. 
		This is a direct representation of overall system efficiency. 
\end{itemize}
Some Important Notes:
\begin{itemize}
	\item The access ratio in the x-axis means $\frac{\text{speed of cores}}{\text{speed of memory}}$
	\item The y-axis on the Trace Execution Graph is in linear scale with time in ns.
	\item In the simulation for Design II, we implement the inter bank coding, however, we have not yet explored the benefit of intra-bank coding introduced in Design II.
	\item The cost of Design II reduces from $2.5 \alpha$, since we don't consider the cost of storing intra bank codes. 
%	\item The cost of 
\end{itemize}
\begin{landscape}
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{\linewidth}
        \includegraphics[width=\linewidth]{LTE.jpg}
\end{minipage}
\caption{
{\bf Performance Graphs for LTE trace} }
\label{fig:LTE}
\end{figure}
%-------------------------------------------------
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
%	\centering
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{LTE_critical_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{LTE_transactional_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{LTE_write_latency_improvement.jpeg}
\end{minipage}
\caption{
{\bf Performance Graphs for LTE trace} }
\label{fig:LTE_improvement}
\end{figure}
%-------------------------------------------------
Observations:
\begin{itemize}
	\item LTE trace is a medium density trace.
	\item The benefit for coding for read access is favourable for access ratios for 4 and more. 
	\item The write transaction latency shows improvement for access ratios of 3 to 6.
	\item The coding benefits are best at access ratio of 4, 5 and 6.
\end{itemize}
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{\linewidth}
        \includegraphics[width=\linewidth]{UMTS.jpg}
\end{minipage}
\caption{
{\bf Performance Graphs for UMTS trace} }
\label{fig:LTE}
\end{figure}
%-------------------------------------------------
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{UMTS_critical_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{UMTS_transactional_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{UMTS_write_latency_improvement.jpeg}
\end{minipage}
\caption{
{\bf Performance Graphs for UMTS trace} }
\label{fig:UMTS_improvement}
\end{figure}
%-------------------------------------------------
Observations:
\begin{itemize}
	\item The UMTS trace is also a medium access trace. 
	\item The read latency improvement in UMTS is substantial for all access ratios in case of critical latency. 
	\item The Transactional Latency improvees untill access ratio of 6.
	\item The design II sees degradation in performance for higher access ratios. 
	\item Write Latency improvement is observed for access ratio of 3 and 4.
	\item The coding benefits are best at access ratio of 4.
\end{itemize}
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{\linewidth}
        \includegraphics[width=\linewidth]{case4.jpg}
\end{minipage}
\caption{
{\bf Performance Graphs for case4 trace} }
\label{fig:case4}
\end{figure}
%-------------------------------------------------
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{case4_critical_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{case4_transactional_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{case4_write_latency_improvement.jpeg}
\end{minipage}
\caption{
{\bf Performance Graphs for case4 trace} }
\label{fig:case4_improvement}
\end{figure}
%-------------------------------------------------
Observations:
\begin{itemize}
	\item The case4 traces are low density traces. That is, the number of access requests per time period are low. 
	\item The Critical Read latency improvement in {\em positive} for all the ratios. 
	\item The critical read latency exponentially improves for increased access ratios.
	\item The transactional Read latency also improves for design I and design III. 
	\item The write latency has only marginal improvement. 
	\item The results suggest that in case4, we do not use the "coding" aspect due to low density access in case of Writes.
	\item The improvement in Transactional Read Latency is substantial. 
\end{itemize}
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{\linewidth}
        \includegraphics[width=\linewidth]{creat4-1.jpg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat4-1 trace} }
\label{fig:creat41}
\end{figure}
%-------------------------------------------------
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{creat4-1_critical_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{creat4-1_transactional_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{creat4-1_write_latency_improvement.jpeg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat4-1 trace} }
\label{fig:creat41_improvement}
\end{figure}
%-------------------------------------------------
Observations:
\begin{itemize}
	\item The trace creat4-1 is a medium density trace. 
	\item The improvement in critical read latency and transactional read latency is significant in design I and design II. 
	\item The write latency is positive till access ratio of 6.
	\item Design I and Design III codes benefit in this trace.
\end{itemize}
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{\linewidth}
        \includegraphics[width=\linewidth]{creat4-2.jpg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat4-2 trace} }
\label{fig:creat42}
\end{figure}
%-------------------------------------------------
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{creat4-2_critical_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{creat4-2_transactional_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{creat4-2_write_latency_improvement.jpeg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat4-2 trace} }
\label{fig:creat42_improvement}
\end{figure}
%-------------------------------------------------
Observations:
\begin{itemize}
	\item This trace is second part of Creat4 trace.creat4-2 is a medium density trace. 
	\item The improvement in critical read latency and transactional read latency is significant in design I and design III. 
	\item The write latency is positive till access ratio of 5.
	\item Design I and Design III codes benefit in this trace.
\end{itemize}
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{\linewidth}
        \includegraphics[width=\linewidth]{creat5-1.jpg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat5-1 trace} }
\label{fig:creat51}
\end{figure}
%-------------------------------------------------
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
	\centering
\begin{minipage}[!t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{creat5-1_critical_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{creat5-1_transactional_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{creat5-1_write_latency_improvement.jpeg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat5-1 trace} }
\label{fig:creat51_improvement}
\end{figure}
%-------------------------------------------------
Observations : 
\begin{itemize}
	\item Creat5-1 is a high density trace. 
	\item There is a significant critical read latency improvement for all access ratios in all design. 
	\item The transactional read latency is improves for all access ratios. 
	\item The write access latency improves for access ratio between 3 and 6.
	\item All the code designs are ideal for this trace. 
	\item Coding architecture is ideal for this trace.
\end{itemize}
\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
\begin{minipage}[!t]{\linewidth}
        \includegraphics[width=\linewidth]{creat5-2.jpg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat5-2 trace} }
\label{fig:creat52}
\end{figure}
%-------------------------------------------------

\cleardoublepage
%-------------------------------------------------
\begin{figure}[htb]
	\centering
\begin{minipage}[!t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{creat5-2_critical_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{creat5-2_transactional_latency_improvement.jpeg}
\end{minipage}
\begin{minipage}[!t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{creat5-2_write_latency_improvement.jpeg}
\end{minipage}
\caption{
{\bf Performance Graphs for Creat5-2 trace} }
\label{fig:creat52_improvement}
\end{figure}
%-------------------------------------------------
Observations : 
\begin{itemize}
	\item Creat5-2 is a part of Creat5 trace. Creat5-2 is a high density trace. 
	\item There is a significant critical read latency improvement for all access ratios in all design. 
	\item The transactional read latency improves for all access ratios.
	\item The write access latency improves for ratios between 3 and 6.
 	\item All the code designs are ideal for this trace. 
	\item Coding architecture is ideal for this trace.
\end{itemize}
\cleardoublepage
{\bf Conclusions}
\begin{itemize}
	\item Table~\ref{table:perfImprovementComparison} summarizes improvement across all traces. 
	\item The systemC simulation of proposed algorithms considers benefit of coding with cost. 
	\item The Coding architecture performs at its best when the trace density is {\em High}. For e.g., Creat5-1 and Creat5-2.
	\item Design I,II and III have associated costs according to table~\ref{table:codedesigncomparison}.
	\item Access Ratio is defined as $\frac{\text{speed of cores in ns}}{\text{speed of memory in ns}}$
\end{itemize}
\begin{table}[tbp]
	\centering
	\begin{tabular}{|c|c|p{4cm}|p{4.2cm}|p{4.2cm}|p{3.3cm}|p{3.3cm}| }
\hline
Trace & Density & Critical Read Latency Improvement & Transactional Read Latency Improvement & Transactional Write Latency Improvement & Access ratio with 15-20$\%$ improvement for Read & Access ratio with 15-20$\%$ improvement for Write\\
% Design & 
\hline
\hline
LTE & Medium &Varies from  -10 to 80$\%$ & Varies from -50 to 80$\%$ & Varies from -150 to 300$\%$ & access ratio 4 to 10 & access ratio 3 to 6 \\
\hline 
UMTS & Medium &Varies from   -5 to 90$\%$ & Varies from 0 to 80$\%$ & Varies from -150 to 150 $\%$ & access ratio 2 to 6 & access ratio 3 to 5 \\
\hline
Case4 & Low &Varies from 1 to 14$\%$ & Varies from -20 to 25$\%$ & Varies from -0.2 to 0.4 $\%$ & access ratio 5 to 10 & None \\
\hline
Creat4-1 & Medium &Varies from 0 to 80$\%$ & Varies from -100 to 80$\%$ & Varies from -15 to 5 $\%$ & access ratio 4 to 10 & access ratio 5 to 6\\
\hline
Creat4-2 & Medium &Varies from -5 to 60$\%$ & Varies from -80 to 60$\%$ & Varies from -17 to 8 $\%$ & access ratio 4 to 10 & None \\
\hline
Creat5-1 & High &Varies from 5 to 95$\%$ & Varies from 5 to 90$\%$ & Varies from -60 to 55 $\%$ & access ratio 2 to 10 & access ratio 3 to 6 \\
\hline
Creat5-2 & High &Varies from 10 to 85$\%$ & Varies from -10 to 90$\%$ & Varies from 10 to 130 $\%$ & access ratio 3 to 10 & access ratio 3 to 10 \\
%\multirow{3}{*}{LTE} & I & 50-90$\%$& & \\
% & II & 50-90$\%$ & 50-90$\%$ & \\
%& III & & & \\
%\multirow{3}{*}{UMTS} & I & & & \\
% & II & & & \\
% & III & & & \\
%\multirow{3}{*}{Case4} & I & & & \\
% & II & & & \\
% & III & & & \\
%Creat4-1 & 0 to 90$\%$ & -30 to 90$\%$ & 15-400 $\%$ \\
%\multirow{3}{*}{Creat4-1} & I & & & \\
% & II & & & \\
% & III & & & \\
%Creat4-2 & 0 to 90$\%$ & -30 to 90$\%$ & 15-400 $\%$ \\
%\multirow{3}{*}{Creat4-2} & I & & & \\
% & II & & & \\
% & III & & & \\
%Creat5-1 & 0 to 90$\%$ & -30 to 90$\%$ & 15-400 $\%$ \\
%\multirow{3}{*}{Creat5-1} & I & & & \\
% & II & & & \\
% & III & & & \\
%Creat5-2 & 0 to 90$\%$ & -30 to 90$\%$ & 15-400 $\%$ \\
%\multirow{3}{*}{Creat5-2} & I & & & \\
% & II & & & \\
% & III & & & \\
\hline
\end{tabular}
\caption{Performance Improvement Comparison Table}
\label{table:perfImprovementComparison}
\end{table}
\end{landscape}
\cleardoublepage
\pagestyle{fancy}


